ReGenesis: LLMs can Grow into Reasoning Generalists via Self-Improvement

Post-training Large Language Models (LLMs) with explicit reasoning trajectories can enhance their reasoning abilities. However, acquiring such high-quality trajectory data typically demands meticulous supervision from humans or superior models, which can be either expensive or license-constrained. In this paper, we explore how far an LLM can improve its reasoning by self-synthesizing reasoning paths as training data without any additional supervision. Existing self-synthesizing methods, such as STaR, suffer from poor generalization to out-of-domain (OOD) reasoning tasks. We hypothesize it is due to that their self-synthesized reasoning paths are too task-specific, lacking general task-agnostic reasoning guidance. To address this, we propose Reasoning Generalist via Self-Improvement (ReGenesis), a method to self-synthesize reasoning paths as post-training data by progressing from abstract to concrete. More specifically, ReGenesis self-synthesizes reasoning paths by converting general reasoning guidelines into task-specific ones, generating reasoning structures, and subsequently transforming these structures into reasoning paths, without the need for human-designed task-specific examples used in existing methods. We show that ReGenesis achieves superior performance on all in-domain and OOD settings tested compared to existing methods. For six OOD tasks specifically, while previous methods exhibited an average performance decrease of approximately 4.6% after post training, ReGenesis delivers around 6.1% performance improvement. We also conduct in-depth analysis of our framework and show ReGenesis is effective across various LLMs and design choices.

==> tables/exp2.tex <==
\begin{table}[t]
\footnotesize
\setlength\tabcolsep{5pt} % default value: 6pt
\caption{Accuracy Results on X math and logical reasoning datasets.}
\label{sample-table}
\begin{center}
\begin{tabular}{l|l|l|cc|c|cc}
\multirow{3}{*}{\bf Domain}&
\multirow{3}{*}{\bf Dataset}&\multirow{1.5}{*}{\bf Training}&\multicolumn{5}{c}{\bf Training data}
\\ \cline{4-8}
&&\multirow{1.5}{*}{\bf Method}&\multicolumn{2}{c|}{\bf Math}&\multicolumn{1}{c}{\bf Logical}&\multicolumn{2}{|c}{\bf Commonsense}
\\ \cline{4-8}
&&&\multicolumn{1}{c}{\bf GSM8K}&\multicolumn{1}{c|}{\bf NumGlue}&\multicolumn{1}{c|}{\bf ARC-c}&\multicolumn{1}{c}{\bf ReClor}&\multicolumn{1}{c}{\bf StrategyQA}\\
\hline
\multirow{10}{*}{Mathematic}&\multirow{5}{*}{ASDIV} & w/o FT 
& $77.2\%$& $77.2\%$& $77.2\%$& $77.2\%$& $77.2\%$\\
&& w/GT& $54.0\%$
&$53.8\%$&$57.7\%$
& $62.0\%$
&$69.4\%$\\
&& LMSI&$77.3\%$&$75.2\%$&$70.9\%$&$77.9\%$&$56.3\%$\\
&& STaR & $79.6\%$&$76.7\%$&$77.0\%$& $76.1\%$&$79.8\%$\\
&&w/ ours&$\mathbf{81.2\%}$&$76.9\%$&$\mathbf{81.6\%}$&$78.3\%$&$\mathbf{81.3\%}$\\
\cline{2-8}
&\multirow{5}{*}{SVAMP} & w/o FT 
& $75.4\%$& $75.4\%$& $75.4\%$& $75.4\%$& $75.4\%$\\
&& w/GT &$40.0\%$ & $54.9\%$ & $57.2\%$ & $56.0\%$ & $72.3\%$\\
&& LMSI&$72.2\%$&$78.2\%$&$72.0\%$&$76.8\%$&$56.8\%$\\
&& STaR &
$71.5\%$
&$76.1\%$
&$76.2\%$&$74.6\%$&$76.2\%$
\\
&&w/ ours&$\mathbf{83.9\%}$&$79.4\%$&$79.5\%$&$76.5\%$&$\mathbf{81.1\%}$\\
\hline 
\multirow{2.5}{*}{Mathematic}&\multirow{5}{*}{AQUA} & w/o FT & $41.3\%$& $41.3\%$& $41.3\%$& $41.3\%$& $41.3\%$\\
&& w/GT &$29.1\%$&$32.3\%$&$18.9\%$&$22.0\%$ & $43.7\%$\\
$\&$&& LMSI
& $31.1\%$
& $40.6\%$
& $32.7\%$
&
&$40.6\%$\\
\multirow{1.5}{*}{Logical}&& STaR 
& $46.9\%$
& $37.0\%$
&$40.6\%$
& $46.1\%$
&$43.3\%$
\\
&&w/ ours 
& $\mathbf{48.8\%}$
& $\mathbf{48.4\%}$
& $\mathbf{46.5\%}$
& $\mathbf{49.6\%}$
& $\mathbf{45.7\%}$
\\
 \hline 
\multirow{5}{*}{Logical}&\multirow{5}{*}{BBH} & w/o FT 
& $60.8\%$& $60.8\%$& $60.8\%$& $60.8\%$& $60.8\%$\\
&& w/GT & $53.6\%$ & $42.4\%$& $37.6\%$ & $44.6\%$ & $52.3\%$
\\
&& LMSI
& $59.5\%$
& $59.5\%$
& $60.8\%$ 
& $53.9\%$
& $60.6\%$
\\
&& STaR 
& $47.4\%$
& $58.5\%$
& $60.7\%$
& $60.6\%$
& $62.9\%$
\\
&&w/ ours 
& $\mathbf{69.3\%}$
& $\mathbf{61.7\%}$
& $\mathbf{66.0\%}$
& $\mathbf{66.8\%}$
&$\mathbf{65.9\%}$
\\
 \hline 
\multirow{5}{*}{NLI}&\multirow{5}{*}{ANLI} & w/o FT 
& $38.4\%$& $38.4\%$& $38.4\%$& $38.4\%$& $38.4\%$\\
&& w/GT & $44.6\%$
& $37.0\%$ & $36.3\%$ & $47.1\%$ & $44.9\%$\\
&& LMSI
& $43.4\%$ 
& $35.1\%$
& $32.5\%$
& $35.1\%$
& $39.8\%$
\\
&& STaR 
& $45.0\%$
& $41.9\%$
& $47.4\%$
& $42.5\%$
& $37.3\%$\\
&&w/ ours
& $43.2\%$
& $50.0\%$
& $50.9\%$
& $44.8\%$
& $\mathbf{55.3\%}$
\\
\end{tabular}
\end{center}
\end{table}
